Dark Matter from Strong Dynamics: The Minimal Theory of Dark Baryons

As a simple model for dark matter, we propose a QCD-like theory based on $\rm{SU}(2)$ gauge theory with one flavor of dark quark. The model is confining at low energy and we use lattice simulations to investigate the properties of the lowest-lying hadrons. Compared to QCD, the theory has several peculiar differences: there are no Goldstone bosons or chiral symmetry restoration when the dark quark becomes massless; the usual global baryon number symmetry is enlarged to $\rm{SU}(2)_B$, resembling isospin; and baryons and mesons are unified together in $\rm{SU}(2)_B$ iso-multiplets. We argue that the lightest baryon, a vector boson, is a stable dark matter candidate and is a composite realization of the hidden vector dark matter scenario. The model naturally includes a lighter state, the analog of the $\eta^\prime$ in QCD, for dark matter to annihilate into to set the relic density via thermal freeze-out. Dark matter baryons may also be asymmetric, strongly self-interacting, or have their relic density set via $3 \to 2$ cannibalizing transitions. We discuss some experimental implications of coupling dark baryons to the Higgs portal.

==> zeromass.tex <==
\section{Massless quark limit}
\label{sec:massless}

To define quark mass on the lattice in a one-flavor theory is not trivial due to the inapplicability of several key properties commonly used.  In this section we use two separate methods to determine the $m_q=0$ limit, and show that the two results are in agreement with each other.
Present experimental and phenomenological constraints do not tell us whether the physical dark quark is massless or not, so for completeness we want to also have the massless limit under numerical control.

\subsection{Axial Ward identity}

Typically the quark mass is evaluated on the lattice by exploiting the axial Ward identity.  In the non-singlet sector, for two mass-degenerate flavours, one writes
\begin{equation}
\langle \partial_tA_t~ \mathcal{O} \rangle = 2 m_q \langle P~ \mathcal{O} \rangle~~,
\label{eq:ward}
\end{equation}
where $A_t$, $P$ and $\mathcal{O}$ are respectively the axial current (temporal component), the pseudoscalar current, and a test current that one is free to choose. Typically $\mathcal{O}=P$, thereby giving a very precise prescription to determine the quark mass $m_q=m_{AWI}$ from fitting a constant to the ratio
\begin{equation}
m_{AWI} = \frac{1}{2}\frac{\langle \partial_tA_t~ P \rangle}{\langle P~ P \rangle}~~.
\label{eq:rward}
\end{equation}
In the singlet case, however, the Ward identity needs to be adjusted to include terms induced by the axial anomaly. As such there is no direct definition of the quark mass by a relation such as Eq.~(\ref{eq:ward}). 
This issue can be circumvented in one-flavor QCD by forming the ratio in Eq.~(\ref{eq:rward}) with a current that includes a mass-degenerate valence fermion $d_{val}$, namely \( P = \bar u \gamma_5 d_{val}\). Essentially one enlarges the symmetry of the valence theory and regains Eq.~(\ref{eq:ward}) as a means to define $m_q$. Within QCD this is a reasonable approximation as the $u$ and $d$ quarks are indeed very light and comparable in mass to each other, with the enlarged symmetry corresponding to a restoration of isospin symmetry.

In the present one-flavor dark matter theory the argument is somewhat more intricate, since the theory does not have a flavor isospin symmetry by definition. Introducing a valence fermion as above does not have a natural analogue and is to be understood as an external fermionic probe. At the same time, the singlet Ward identity picks up the extra anomaly-induced terms.
To illustrate, we show the ratio of Eq.~(\ref{eq:rward}) calculated by using only the connected (left panel) or combined (right panel) currents in Fig.~\ref{fig:awis}.  The connected calculation corresponds to using the $\pi$ meson (not physically present in our one-flavour theory).
The combined calculation corresponds to using the $\eta$ meson of our theory.

\begin{figure}[h!]
%\centering
\includegraphics[width=0.49\textwidth]{./figures/nf1_awi_conn.png}
\includegraphics[width=0.49\textwidth]{./figures/nf1_awi.png}
\caption{The quark mass obtained from the axial Ward identity, Eq.~(\ref{eq:rward}), with connected (left panel) or connected and disconnected (right panel) contributions.}
\label{fig:awis}
\end{figure}

While the non-singlet calculation yields flat behavior as one would expect, the singlet results show a strong rise in the data towards the mid point.
We anticipate that the singlet can be separated into a sum of connected and disconnected pieces and, given the relative sizes of the error bars, we define the quark mass from the non-singlet Ward identity calculated using a mass-degenerate valence fermion. 
Extrapolation of the data from the left panel of Fig. 6 leads to $m_\pi=0$ when the bare mass takes a critical value of
\begin{equation}\label{eq:mc}
m_c=-0.901(9) \,.
\end{equation}

